A Framework for Enriching Lexical Semantic Resources with Distributional Semantics

We present an approach to combining distributional semantic representations induced from text corpora with manually constructed lexical-semantic networks. While both kinds of semantic resources are available with high lexical coverage, our aligned resource combines the domain specificity and availability of contextual information from distributional models with the conciseness and high quality of manually crafted lexical networks. We start with a distributional representation of induced senses of vocabulary terms, which are accompanied with rich context information given by related lexical items. We then automatically disambiguate such representations to obtain a full-fledged proto-conceptualization, i.e. a typed graph of induced word senses. In a final step, this proto-conceptualization is aligned to a lexical ontology, resulting in a hybrid aligned resource. Moreover, unmapped induced senses are associated with a semantic type in order to connect them to the core resource. Manual evaluations against ground-truth judgments for different stages of our method as well as an extrinsic evaluation on a knowledge-based Word Sense Disambiguation benchmark all indicate the high quality of the new hybrid resource. Additionally, we show the benefits of enriching top-down lexical knowledge resources with bottom-up distributional information from text for addressing high-end knowledge acquisition tasks such as cleaning hypernym graphs and learning taxonomies from scratch.

==> glossary.tex <==
\section*{Glossary}

\begin{enumerate}

\item \textbf{Semantification}. The process through which instances of lexical units (i.e., single- or multi-word expressions) from an arbitrary resource (e.g., text or extraction triples) are labeled with an explicit symbol that uniquely identifies their specific meaning (we refer to such meaning also as `concept' or `sense' interchangeably throughout the paper). For instance, in the vision of the Semantic Web \cite{bernerslee2001semantic} this amounts to associating instances of potentially ambiguous content words and proper names with unambiguous URIs. In the field of NLP this can viewed as equivalent to the `classic' task of Word Sense Disambiguation \cite{Navigli2009} or, in the case of named entities, Entity Linking (see below).

\item \textbf{Uniform Resource Identifier (URI)} / \textbf{URIfied}. A Uniform Resource Identifier (URI) is a string of characters used to identify an abstract or physical resource \cite{hitzler09}. In the vision of the Semantic Web and, in particular, in the Linked Open Data Cloud \cite{bizer09b}, URIfied is a technical term to refer to all those resources where each piece of information has a unique Uniform Resource Identifier.

\item \textbf{Knowledge Base (KB)} / \textbf{Knowledge Graph (KG)}. Knowledge bases have a long history in the field of AI \cite{buchanan05,buchanan06}. In general, KBs can be viewed as repositories of structured information providing an explicit representation of knowledge about one or more domains of interest -- that is, our generic use of the term encompasses lexical semantic networks like WordNet all the way through databases of relational statements like DBpedia or WikiData. KBs overlap with ontologies \cite{guarino09}, which provide a formal model of the relevant entities and relations pertaining to the structure of a system. Most popular knowledge bases like WordNet, DBpedia or BabelNet can be viewed as graphs where the nodes describe entities and captures semantic relations between them. Accordingly, we refer to KBs interchangeably as Knowledge Graphs (KGs), which are, in fact, graph-based representations of a KB. Much research efforts concentrated in the past years on building KBs from the content of collaboratively generated resources such as Wikipedia \cite{hovy13a}: we refer to these resources as \textbf{encyclopedic-centric} in that they essentially rely on the vocabulary of entities provided by the `the free encyclopedia that anyone can edit'.

\item \textbf{Entity Linking}: The task of matching mentions of named entities in text with unique identifiers (e.g., URIs) such as those provided by a reference Knowledge Base -- e.g., any of DBpedia, BabelNet or Wikidata that are essentially derived from semi-structured information found in Wikipedia \cite{mihalcea07}. Entity Linking roughly corresponds to the long-standing task of Word Sense Disambiguation (WSD), but with an additional focus on the sense/entity vocabulary provided by an external KB, i.e., named entities like Person, Location, Organization, Miscellaneous artefacts, etc.

\item \textbf{Open and Closed Information extraction (IE)}. We define IE generically as the task of automatically extracting structured information from unstructured and/or semi-structured machine-readable documents -- e.g., raw text. In our discussions we rely on the distinction first introduced by \cite{banko07} of `open' vs. `closed' information extraction systems. Open IE systems, in contrast to closed ones, do not rely on a pre-defined schema or set of semantic relations of interest that needs to be specified in advance.

\end{enumerate}

